Multi-Objective Approaches to Markov Decision Processes with Uncertain Transition Parameters

Markov decision processes (MDPs) are a popular model for performance analysis and optimization of stochastic systems. The parameters of stochastic behavior of MDPs are estimates from empirical observations of a system; their values are not known precisely. Different types of MDPs with uncertain, imprecise or bounded transition rates or probabilities and rewards exist in the literature. Commonly, analysis of models with uncertainties amounts to searching for the most robust policy which means that the goal is to generate a policy with the greatest lower bound on performance (or, symmetrically, the lowest upper bound on costs). However, hedging against an unlikely worst case may lead to losses in other situations. In general, one is interested in policies that behave well in all situations which results in a multi-objective view on decision making. In this paper, we consider policies for the expected discounted reward measure of MDPs with uncertain parameters. In particular, the approach is defined for bounded-parameter MDPs (BMDPs) [8]. In this setting the worst, best and average case performances of a policy are analyzed simultaneously, which yields a multi-scenario multi-objective optimization problem. The paper presents and evaluates approaches to compute the pure Pareto optimal policies in the value vector space.

==> document.tex <==
\section{Mathematical Preliminaries}
\label{sec:Preliminaries}


==> theoretical-considerations.tex <==
\section{Theoretical considerations}
\label{sec:theory}

Prior to discussing practical algorithms, we would like to establish
some complexity results about multi-objective optimization for BMDPs.
These will allow us, first, to constrain the algorithmic possibilities,
and second, to clearly define optimization goals.

\subsection{Solutions with guaranteed performance}
\label{sec:hardness}

We first consider the \emph{canonical decision} problem. Informally, it
consists of finding a policy that meets given minimum performance 
bounds.

\begin{definition}[Canonical decision problem]
  Given a vector $\vec{u} \in \R^c$ and a multi-objective optimization
problem in a general form
\[ 
  \max_{\vec x \in X} f_1(\vec{x}), f_2(\vec{x}), \ldots, f_c(\vec{x}),
\]
the \emph{canonical decision problem} is defined to decide, if a vector
$\vec{x}^*$ such that $\vec{x}^* \in X$ and $f_j(\vec{x}^*) \ge u_j$ for
all $j \in [c]$ exists.
\end{definition}

In the context of BMDPs solving the canonical decision problem would 
mean to find, given vectors $\vec{u}_\downarrow, \overline{\vec{u}}, 
\vec{u}_\uparrow$, a policy $\pi$ such that the worst case, expected, 
and best case value vectors $\vec{v}_\downarrow^{(\pi)}, 
\overline{\vec{v}}^{(\pi)}, \vec{u}_\uparrow^{(\pi)}$ under $\pi$ are at 
least as large as the respective bounds $\vec{u}_\downarrow, 
\overline{\vec{u}}, \vec{u}_\uparrow$. It has been shown by 
\cite{DBLP:conf/stacs/ChatterjeeMH06} that the corresponding decision
problem is \NP-hard for general multi-objective MDPs where different
expected values are computed. The following theorem shows that the
hardness result also holds for SBMDPs even if rewards do not depend on
the chosen action and even if we consider only two objectives.

\begin{theorem}
\label{thm:pareto-nphard}
  Deciding existence of a pure policy $\pi$ for a given stochastic
bounded-parameter Markov decision process that delivers a worst-case
expected discounted reward $\vec v_{\downarrow}^{(\pi)}$ and an
average-case expected discounted reward $\overline{\vec v}^{(\pi)}$
such that $\vec{v}_{\downarrow}^{(\pi)} \ge \vec{v}_1,
\overline{\vec{v}}^{(\pi)} \ge \vec v_2$ for given vectors $\vec{v}_1,
\vec{v}_2$ is \NP-complete.
\end{theorem}

We would like to note that this result also applies to other
multi-objective measures, such as the combination of best-case and
expected-case measures, and best-case and worst-case measures.
%\end{comment}

\ifthenelse{\boolean{complexity}}{%
\subsection{Pareto optimality measures}
\label{sec:pareto-hardness}

By generalizing the considered problem as a variant of a multi-objective
Markov decision process problem, with the components being the
worst-case, best-case, or average-case expected discounted rewards, we
can consider general measures for optimality in multi-objective
optimization problems. Hence, it is tempting to consider known
techniques for multi-objective optimization in this context.
}{}

% For a given weight vector, Algorithm~\ref{alg:scalarization} describes 
% a variant of value iteration which converges to an optimal pure policy. 
% We denote the corresponding policy as $\pi^{\vec w}$. However, if $\vec 
% w$ is not known a priori, one is usually interested in the complete set 
% of pure policies which are optimal for some weight vector. More 
% formally, let $\mathcal{W} = \{ \vec w = (w_\downarrow, \overline{w}, 
% w_\uparrow) \mid \vec w \ge \vec 0, \vec w \idvt = 1\}$ the set of 
% weight vectors and let $\Ppure$ be the set of pure policies. Then define
% \[
% \Pweight = \left\{\pi \mid \pi \in \Ppure,
% \exists \vec
% w \in \mathcal{W}: \pi = \pi^{\vec w}\right\}
% \]
% as the set of pure policies that are optimal for some weight vector.

% Furthermore, it is easy to see that the vectors in $\Vweight$ span the 
% convex hull of $\Vpure$. Nevertheless, the number of policies in 
% $\Pweight$ can still be exponential in the size of the MDP.

\ifthenelse{\boolean{nonstationary}}{%
Up to now we have only considered optimal stationary policies and in
our setting pure policies are of special importance. However, if we
allow general policies which consider the history, then additional
Pareto optimal solutions may be found. This will be shown by a simple
example (shown in Fig.~\ref{ex:simple}). The SBMDP has two states,
in state $1$ one can choose between action $a$ and $b$. If $a$ is
selected the process goes with probability $p$, which is uniformly $[0,1]$
distributed, into state $2$ and stays with probability $1-p$ in state
$1$. If $b$ is selected, then the process makes with probability $q$,
which is uniformly $[0.5,0.7]$ distributed, a transition to state $2$
and stays with probability $1-q$ in state $1$. From state $2$ the
process always returns to state $1$ with probability $1$ no matter
which action has been chosen.  The reward vector is $\vec{r}^a =
\vec{r}^b = {(1, 0)}^\top$. 

\begin{figure}[htp]
    \centering
    \begin{tikzpicture}[auto,>=stealth',node distance=2cm]
      \node[circle,draw] (1) at (0,3) {$1$};
      \node[circle,draw] (2) at (2,0) {$2$};
      
      \path[->] (1) edge [bend left=60] node {a$[0,1]$, b$[0.5,0.7]$} (2);      
      \path[->] (2) edge [bend right=-60] node {*$[1,1]$} (1);
      \path[->] (1) edge [loop left=90] node {a$[0,1]$, b$[0.3,0.5]$} (1);
 
  \end{tikzpicture}
  \caption{Simple example SBMDP}
\label{ex:simple}
\end{figure}

Since decisions in state $2$ are irrelevant, we have two pure policies
namely $(a)$ which chooses always action $a$ and $(b)$ that chooses
always $b$. Obviously, $(a)$ is better for maximizing the average 
reward and $b$ is better for the worst case reward. For $\gamma=0.9$ the corresponding
values are $\vec{v}_1^{(a)} = \left(v_{1
    \downarrow}^{(a)}, \overline{v}_1^{(a)}, v_{1\uparrow}^{(a)}\right) = \left(5.2632,
  6.8966, 10.000\right)$ and  
$\vec{v}_1^{(b)} = \left(v_{1 \downarrow}^{(b)}, \overline{v}_1^{(b)},
v_{1 \uparrow}^{(b)}\right) =
\left(6.1350, 6.4935, 6.8966\right)$. Both vectors
are Pareto optimal. Now consider the non-stationary polices $ab$ and
$ba$ which collect alternating sequences of the actions $a$ and
$b$ in state $1$. We have $\vec{v}_1^{(ab)} = \left(v_{1 \downarrow}^{(ab)},
  \overline{v}_1^{(ab)},v_{1 \uparrow}^{(ab)}\right) = \left(5.2632,
  6.7024, 7.8684\right)$ and 
$\vec{v}_1^{(ba)} = \left(v_{1 \downarrow}^{(ba)},
  \overline{v}_1^{(ba)}, v_{1 \uparrow}^{(ba)}\right) = \left(5.5913,
  6.6398, 7.6316\right)$. $\vec v_1^{(ab)}$ is dominated by
  $\vec{v}_1^{(a)}$ whereas $\vec v_1^{(ba)}$ is another Pareto optimal
  vector which cannot be reached with any stationary policy. By
extending the history, we obtain additional Pareto optimal
policies. Figure~\ref{fig0} shows the Pareto optimal value vectors for state $1$
according the minimum and maximum which have been computed with the
algorithm presented below. For an relative error of $0.001$, $155$
Pareto optimal value vectors are computed for the minimum and maximum
and $428$ Pareto optimal vectors considering all three goals, minimum,
maximum and average value. 

\begin{figure}
  \centering
  \includegraphics[width=118mm]{First.pdf} 
  \caption{Pareto optimal values for the gain of state $1$ in the
    simple example.}
\label{fig0}
\end{figure}

We define $\Popt$ as the set of Pareto optimal policies. In general, 
$\Popt$ can be an infinite set but since decisions $k$ steps apart 
receive a discounting factor $\gamma^k$, the influence of past decisions 
vanishes exponentially. Again we denote by $\Vopt$ the set of value 
vectors belonging to policies from $\Popt$.
}{}


